Primitive Integral Solutions to x^2 + y^3 = z^{10}

We classify primitive integer solutions to x^2 + y^3 = z^10. The technique is to combine modular methods at the prime 5, number field enumeration techniques in place of modular methods at the prime 2, Chabauty techniques for elliptic curves over number fields, and local methods.

==> code/allCode <==
//////////////////////////////////////////////////////////////////
// Computations were done using Magma, version V2.13-6
//////////////////////////////////////////////////////////////////

///////////////////////////////////////////////////////////////////////
// This Magma code constructs the object of sections 3 and 4 of
// "Primitive integral solutions to X^2 + y^3 = z^10" by David Brown
//
// These are necessary for the elliptic Chabauty computation of section 5
// and is called by the other MAGMA routines.
///////////////////////////////////////////////////////////////////////

QQ := Rationals();
ZZ := Integers();
P<t> := PolynomialRing(QQ);


//////////////////////////////////////////////////////////////////////
// This is the defining polynomial of the number field K_j
//////////////////////////////////////////////////////////////////////

    fj :=  (t^2 + 250*t + 3125)^3  - j*t^5;


    //////////////////////////////////////////////////////////////////////
    // Need to factor because in the CM case fj may not be irreducible.
    // In the j = 12^3 case there are multiple isogenies, defined over different
    // fields. The second choice of field gives a curve of rank 0.
    //////////////////////////////////////////////////////////////////////

    Fj := j eq 12^3 select Factorization(fj)[2][1]
        else Factorization(fj)[1][1];


    //////////////////////////////////////////////////////////////////////
    // This creates the number field K_j 
    //
    // An elliptic curve E with j(E) = j has a 5 isogeny over this field.
    //////////////////////////////////////////////////////////////////////

    Kj := NumberField(Fj);

//////////////////////////////////////////////////////////////////////
// This creates the elliptic curve X_{E_0} over QQ and
// for a given j creates it over K_E
//////////////////////////////////////////////////////////////////////

EQ<x,y,z> := EllipticCurve(t*(t^2  + (-3)*22*t +(-3)^2*125));
Ej := BaseExtend(EQ,Kj);


    //////////////////////////////////////////////////////////////////////
    // This creates the canonical point on X_E_0(K_E) coming from the 
    // 5-isogeny of E over K_j. 
    //
    // For this to work j(E) must be in the image of -3z^2 + 12^3
    //////////////////////////////////////////////////////////////////////

    bool, z0 := IsSquare((j-12^3)/(-3));
    if bool then
      canPts :=  {@Ej![ -3*Kj.1, 9*z0*Kj.1^3/p1 ,1]
          where p1 is Evaluate(t^2 - 500*t - 15625, Kj.1)@};
      else
          canPts := {@@};
    end if;


//////////////////////////////////////////////////////////////////////
// Create the map X_E_0 \to X_E_0,Delta
//-- extend the map to cover pts at infty etc TODO
//////////////////////////////////////////////////////////////////////

    P1<Z,W> := ProjectiveSpace(Rationals(),1);
    jp0 := map< EQ -> P1 | [-3*y*(X^2 - 500*X*z - 15625*z^2), x^3  ] 
    	   where X is x/-3  >;
    jp0 := Extend(jp0);


    //////////////////////////////////////////////////////////////////////
    // Base Extend to K_j
    //-- Extend the map to cover .. TODO
    //////////////////////////////////////////////////////////////////////

    P1j<Z,W> := ProjectiveSpace(Kj,1);
    jp := map< Ej -> P1 | [ -3*y*(X^2 - 500*X*z - 15625*z^2), x^3  ] 
       	    where X is x/-3  >;
    jp := Extend(jp);

    //////////////////////////////////////////////////////////////////////
    // Create the map X_E_0,Delta \to X(1)
    //////////////////////////////////////////////////////////////////////

    sp := map<P1 -> P1 | [-3*Z^2 + 12^3*W^2, W^2]>;
    sp := Extend(sp);

//////////////////////////////////////////////////////////////////////
// Create the MWmap
//////////////////////////////////////////////////////////////////////

G := AbelianGroup([6,0]);
gs := [Ej![45 , 90 , 1] , canPts[1]] ; 
mwMap := map<G->Ej|g:->&+[c[i]*gs[i]:i in [1..#gs]] where c:=Eltseq(g)>;





////////////////////////////////////////////////////////////////////
// This Magma code does the elliptic Chabauty computations necessary
// for section 5 of  "Primitive integral solutions to X^2 + y^3 = z^10" 
// by David Brown, in the case of j = 0
////////////////////////////////////////////////////////////////////

////////////////////////////////////////////////////////////////////
// Construct the number fields, curves, maps, etc necessary.
////////////////////////////////////////////////////////////////////

j := 0;
//load "chabautyNecessities";


////////////////////////////////////////////////////////////////////
// Do a two descent.
////////////////////////////////////////////////////////////////////

// Uncomment this to do it yourself.
//RankBound(Ej); // Returns 1


////////////////////////////////////////////////////////////////////
// Do the elliptic Chabauty computation. 
// 7 is the first prime that works.
////////////////////////////////////////////////////////////////////

p := 19; 
bound, found, index, cosets := Chabauty(mwMap,jp,p : Aux := {13});

    // bound returns 10
    // found returns 10
       found := SetToIndexedSet(found);
    // index returns 2



////////////////////////////////////////////////////////////////////
// Since the index is 40. We need to check that G \subset  E(K) has 
// index coprime to 40
////////////////////////////////////////////////////////////////////

    ////////////////////////////////////////////////////////////////////
    // Check 2-saturation
    // Q is the canonical point of infinite order
    // T is the non-trivial two torsion point
    // 
    // We don't need to worry about 3-torsion because 5 is prime to 3
    ////////////////////////////////////////////////////////////////////


    {#DivisionPoints(P,2)
        where P is a*Q + b*T
        where Q is gs[2]
        where T is 3*gs[1]:
        a in [1..1], b in [0..1] };
	  
    // Returns {0}, so G is 2-saturated


////////////////////////////////////////////////////////////////////
// Check the images of the found points and see if they correspond 
// to primitive solutions to x^2 + y^3 = z^10
////////////////////////////////////////////////////////////////////

images := {@ sp(jp(mwMap( pt ))) : pt in found @};

    // returns no new j Invariants.

bound;

////////////////////////////////////////////////////////////////////
// This Magma code does the elliptic Chabauty computations necessary
// for section 5 of  "Primitive integral solutions to X^2 + y^3 = z^10" 
// by David Brown, in the case of j = 1728
////////////////////////////////////////////////////////////////////

////////////////////////////////////////////////////////////////////
// Construct the number fields, curves, maps, etc necessary.
////////////////////////////////////////////////////////////////////

j := 1728;
//load "chabautyNecessities";


////////////////////////////////////////////////////////////////////
// Do a two descent.
////////////////////////////////////////////////////////////////////

// Uncomment this to test
// RankBound(Ej); // Returns 0


////////////////////////////////////////////////////////////////////
// There are twelve torsion points.
////////////////////////////////////////////////////////////////////

tors, m := TorsionSubgroup(Ej);
  #tors;	    // returns 12

tors := {@m(pt) : pt in tors@};

////////////////////////////////////////////////////////////////////
// Check the images of the found points and see if they correspond 
// to primitive solutions to x^2 + y^3 = z^10
////////////////////////////////////////////////////////////////////

images := {@ sp(jp( pt )) : pt in tors @};

    // Returns no new j-invariants.



////////////////////////////////////////////////////////////////////
// This Magma code does the elliptic Chabauty computations necessary
// for section 5 of  "Primitive integral solutions to X^2 + y^3 = z^10" 
// by David Brown, in the case of j = -13824
////////////////////////////////////////////////////////////////////

////////////////////////////////////////////////////////////////////
// Construct the number fields, curves, maps, etc necessary.
////////////////////////////////////////////////////////////////////

j := -13824;
//load "chabautyNecessities";


////////////////////////////////////////////////////////////////////
// Do a two descent.
////////////////////////////////////////////////////////////////////

// Uncomment this to test.
// RankBound(Ej); // Returns 1


////////////////////////////////////////////////////////////////////
// Do the elliptic Chabauty computation. 
// 7 is the first prime that works.
////////////////////////////////////////////////////////////////////

p := 7; 
bound, found, index, cosets := Chabauty(mwMap,jp,p);

    // bound returns 8
    // found returns 8
       found := SetToIndexedSet(found);
    // index returns 40



////////////////////////////////////////////////////////////////////
// Since the index is 40. We need to check that G \subset  E(K) has 
// index coprime to 40
////////////////////////////////////////////////////////////////////

    ////////////////////////////////////////////////////////////////////
    // Check 2-saturation
    // Q is the canonical point of infinite order
    // T is the non-trivial two torsion point
    // 
    // We don't need to worry about 3-torsion because 5 is prime to 3
    ////////////////////////////////////////////////////////////////////


    {#DivisionPoints(P,2)
        where P is a*Q + b*T
        where Q is gs[2]
        where T is 3*gs[1]:
        a in [1..1], b in [0..1] };
	  
    // Returns {0}, so G is 2-saturated
    
    ////////////////////////////////////////////////////////////////////	
    // Check 5-saturation
    // Only need to check P because 5 is prime to the order of the torsion
    ////////////////////////////////////////////////////////////////////

    #DivisionPoints(Q,5)
	where Q is gs[2];

    // Returns 0, so G is 5-saturated.

////////////////////////////////////////////////////////////////////
// Check the images of the found points and see if they correspond 
// to primitive solutions to x^2 + y^3 = z^10
////////////////////////////////////////////////////////////////////

images := {@ sp(jp(mwMap( pt ))) : pt in found @};

    // returns no new j Invariants.


///////////////////////////////////////////////////////////////
// This routine runs the Chabauty computations indicated at the 
// in the `reducible level lowering at 2' lemma of the paper 
// Primitive integral solutions to x^2 + y^3 = z^10 by 
// David Brown.
///////////////////////////////////////////////////////////////

P<t> := PolynomialRing(Rationals());

// Case when v,v^2 + 3u^2 are coprime


f1 := t^5 - 3^5;
H1 := HyperellipticCurve(f1);
pts1 := RationalPoints(H : Bound := 1000);
J1 := Jacobian(H1);
RankBound(J1); // Returns 0, so we are done.


// Case when v,v^2 + 3u^2 are not coprime
// So that 3 exactly divides v^2 + 3*u^2


f2 := t^5 - 3^7;
H2 := HyperellipticCurve(f2);
pts2 := RationalPoints(H2 : Bound := 1000);
J2 := Jacobian(H2);
RankBound(J2); // Returns 1, so we must Chabauty.

Jpts := RationalPoints(J2 : Bound := 5000);
pt := Jpts[2];
Order(pt); // Infinite order.


// See Magma example H113E25
LogarithmicBound := Height(pt) + HeightConstant(J2 : Effort := 2, Factor);  
AbsoluteBound := Ceiling(Exp(LogarithmicBound));
  // The next step takes a few minutes..		  
PtsUpToAbsBound := Points(J2 : Bound:=AbsoluteBound );
ReducedBasis( [ pt : pt in PtsUpToAbsBound ]);
  // Returns that pt generates 
pt := ReducedBasis[1];
Chabauty(pt,17); // Returns {}

//////////////////////////////////////////////////////////////////
// This code shows that all Number Fields unramified away from
// {2,3} are two torsion fields of elliptic curves.
//
// This computations are relevant for the `level lowering at 2'
// remark the paper "Primitive Integral Solutions to x^2 + y^3
// = z^{10}' by David Brown
//////////////////////////////////////////////////////////////////

P<x> := PolynomialRing(Rationals());


//////////////////////////////////////////////////////////////////
// Computed the following using sage
// J = JonesDatabase()
// J.unramified_outside([2,3])
//////////////////////////////////////////////////////////////////
f := [x^3 - 3*x + 1, x^3 - 2, x^3 + 3*x - 2, x^3 - 3, x^3 - 3*x - 4, x^3 - 3*x - 10, x^3 - 12, x^3 - 6, x^3 - 9*x - 6];
K := [NumberField(g) : g in f];

//////////////////////////////////////////////////////////////////
// This gets all elliptic curves of conductor dividing 12^3
//////////////////////////////////////////////////////////////////

D := CremonaDatabase();
e := {@@};
for a in [0..3] do
  for b in [0..6] do
    e := e join {@E : E in EllipticCurves(D,2^a*3^b)@};
  end for;
end for;

g := {@ HyperellipticPolynomials( WeierstrassModel(E)) : E in e@};;


//////////////////////////////////////////////////////////////////
// For each number field k in K, this searches for an elliptic
// curve with two torsion field isomorphic to k
//
// (It returns that all 9 k in K are two torsion fields.)
//////////////////////////////////////////////////////////////////

K_low := [k : k in K | exists{f : f in g | IsIrreducible(f) and  IsIsomorphic(k,NumberField(f))}];


//////////////////////////////////////////////////////////////////
// This picks out a single E for each k in K
//////////////////////////////////////////////////////////////////

pairs := {@@};
for k in K do
        bool := exists(t){f : f in g | IsIrreducible(f) and  IsIsomorphic(k,NumberField(f))};
        pairs := pairs join {<k,t>};
end for;



/////////////////////////////////////////////////////////////////////
// This code creates the elliptic curves used in the computations 
// of `Primitive Integral Solutions to x^2 + y^3 = z^10' by David
// Brown
/////////////////////////////////////////////////////////////////////

  /////////////////////////////////////////////////////////////
  // Query Magma's Cremona Database and get the curves 
  // described in Section 4.
  /////////////////////////////////////////////////////////////

  D := CremonaDatabase();

  conds := {@ "24A1"," 27A1"," 32A1"," 36A1"," 54A1"," 96A1"," 108A1"," 216A1"," 216B1"," 288A1", 
  	      "864A1"," 864B1"," 864C1" @};

  crvs := {@ EllipticCurve(D, "24A1"), EllipticCurve(D,"27A1"), EllipticCurve(D,"32A1"), 
       	     EllipticCurve(D,"36A1"), EllipticCurve(D,"54A1"), EllipticCurve(D,"96A1"),	
	     EllipticCurve(D,"108A1"), EllipticCurve(D,"216A1"), EllipticCurve(D,"216B1"), 
	     EllipticCurve(D,"288A1"), EllipticCurve(D,"864A1"), EllipticCurve(D,"864B1"), 
	     EllipticCurve(D,"864C1") @};

  jInvs := {@jInvariant(c) : c in crvs@};


  /////////////////////////////////////////////////////////////
  // Collect the curves which are non-CM.
  // (These we can handle without local methods)
  /////////////////////////////////////////////////////////////

  crvsGood := {@c : c in crvs | not jInvariant(c) in {0,12^3}@};
  jInvsGood := {@j : j in jInvs | not j in {0,1728} @};

  /////////////////////////////////////////////////////////////
  // Collect the curves such that X_E(5) is not isomorphic to 
  // the Symplectic Twist X_{E^{-1}}(5).
  /////////////////////////////////////////////////////////////  

  crvsAnti := {@ EllipticCurve(D,"216A1"), 
	      	 EllipticCurve(D,"216B1"), 
 	   	 EllipticCurve(D,"864A1"), 
	   	 EllipticCurve(D,"864B1"), 
	   	 EllipticCurve(D,"864C1") @};

///////////////////////////////////////////////////////
// This code creates the explicit equations for the maps 
// X_E(N) \to X(1) necessary for the 
// local tests of section 6 of the paper `Primitive
// Integral Solutions to x^2 + y^3 = z^10' by David
// Brown
///////////////////////////////////////////////////////

QQ := Rationals();
ZZ := Integers();
P<t> := PolynomialRing(QQ);

//load "local_1_get_elliptic_curves";


////////////////////////////////////////////////////////////////
// INPUT: an elliptic curve c and an integer N
//
////////////////////////////////////////////////////////////////
// OUTPUT: The (affine piece of) the map X_c(N) to P^1  
// 	   (Symplectic case)
////////////////////////////////////////////////////////////////

getjInvSymp := function(c,N)
	////////////////////////////////////////////////////////
	// This gets the input to the RubSilv rouutine
	////////////////////////////////////////////////////////

	j := jInvariant(c);
	J := j/12^3;

	eqn := Coefficients(WeierstrassModel(c));
	A := eqn[4];
	B := eqn[5];

	////////////////////////////////////////////////////////
	// Get the X_E(N) \to X(1) equations
	////////////////////////////////////////////////////////
	a,b := RubinSilverbergPolynomials(N,J);

	////////////////////////////////////////////////////////
	// Make the universal elliptic curve, with parameter T
	////////////////////////////////////////////////////////
	P := Parent(a);
	Q<T> := FieldOfFractions(P);

	e := EllipticCurve([A*Q!a,B*Q!b]);

	////////////////////////////////////////////////////////
	// get the universal j-invariant 
	////////////////////////////////////////////////////////
	j := jInvariant(e);

	////////////////////////////////////////////////////////
        // Break it up
	////////////////////////////////////////////////////////
	num := Numerator(j);
	den := Denominator(j);	

	return j, num, den;
end function;



//////////////////////////////////////////////////////////////
// Helper routines for computing equations for the 
// anti-symplectic twist X_c(N)^- \to X(1)
//////////////////////////////////////////////////////////////

//////////////////////////////////////////////////////////////
// 1) Compute a number field K such that 
//    E has an isogeny over K
//////////////////////////////////////////////////////////////

twoIsogenyPolynomial := function(c)
	j := jInvariant(c);
	phi := AtkinModularPolynomial(2);
	return Evaluate(phi,[t,j]);
end function;


twoIsogenyField := function(c)
	j := jInvariant(c);
	phi := AtkinModularPolynomial(2);
	return K, K.1 where K is NumberField(f) where f is Factorization(Evaluate(phi,[t,j]))[1][1];
end function;


///////////////////////////////////////////////////
// Subroutine *Mobius*: 
//  Input: two triples of points in A^1
//  Output: the corresponding map P^1 to P^1
//  (the affine polynomial at least)
///////////////////////////////////////////////////

mobius := function(e,j)
     M := Matrix(3,4,
       [[e[1],1,-j[1]*e[1],-j[1]],
        [e[2],1,-j[2]*e[2],-j[2]],
        [e[3],1,-j[3]*e[3],-j[3]] ]
     );
     
     b := Basis(NullspaceOfTranspose(M))[1];
       P<t> := PolynomialRing(BaseRing(Parent(b)));
     return (b[1]*t + b[2])/(b[3]*t + b[4]);
end function;


///////////////////////////////////////////////////
// getAntiSymplectic:
///////////////////////////////////////////////////
// Input: elliptic curve c, an integer N. 
//	    		    (only N = 5 is implemented)
// Output: equations for the anti-symplectic twist
// 	   X_c'(N) of X(N)  
///////////////////////////////////////////////////

///////////////////////////////////////////////////
// Antisymplectic case
///////////////////////////////////////////////////
// The pre-computed polys are in the file `saved polys' under
// the name antiSympPolys; 
////////////////////////////////////////////////////////////

//restore "savedPolys"; // Uncomment this line if using 
	  		// precomputed polynomials.
antiSympPolys := [];    


getjInvAntiSymp :=  function(c : preCompute := false) 
    P<T> := PolynomialRing(Rationals());

  if not preCompute then

    //////////////////////////////////////////////////    
    // Get (and match up) the two torsion and 
    // two isogenies.
    //////////////////////////////////////////////////
    j := jInvariant(c);	      

    f := HyperellipticPolynomials(c);
        K := SplittingField(f);	      	      
	Q<t> := PolynomialRing(K);
	e := BaseExtend(c,K);
    F := Q!f;
        roots    := [r[1] : r in Roots(F)];
    	twoTors  := [e![r,0,1] : r in roots];
	twoIsogs := [TwoIsogeny(i) : i in twoTors];
	jInvsIsog := [jInvariant(Codomain(phi)) : phi in twoIsogs];
	
    //////////////////////////////////////////////////
    // Construct the canonical points on X_F(5), 
    // where F is the first isogenous curve
    //
    // Also, MAGMA v.2.13.6 has coercion issues... 
    //////////////////////////////////////////////////
    j,n,d := getjInvSymp(Codomain(twoIsogs[1]) , 5);
    canPts := {@0@};
	   _,can2 := HasRoot(n - jInvsIsog[2]*d);
	   	  _,m := IsIsomorphic(Parent(can2),K);
		  can2 := m(can2);	  
	     canPts := canPts join {@can2@};
	   _,can3 := HasRoot(n - jInvsIsog[3]*d);
	   	  _,m := IsIsomorphic(Parent(can3),K);
		  can3 := m(can3);
	     canPts := canPts join {@can3@};	   	      


    jQ :=  Evaluate(j,mobius(roots,canPts));
    return P!Numerator(jQ)/P!Denominator(jQ);

  else
    if exists(i){i : i in [1..#crvsAnti] | IsIsomorphic(c,crvsAnti[i])} 
    then
       return antiSympPolys[i];
    else
	return "Nothing precomputed for this curve";
    end if;
  end if;    	   
end function;


///////////////////////////////////////////////////////////////
// getjInvs -- auxiliary function combining the symp and anti 
// 	       symplectic cases.
///////////////////////////////////////////////////////////////

getjInv := function(c,N : anti := false, preCompute := true)
  return not anti select getjInvSymp(c,N)
  	 else getjInvAntiSymp(c : preCompute := preCompute);	 
end function;



///////////////////////////////////////////////////////////////
// This collects the (factors of the) homogeneous 
// polynomials defining the map X_c(N) \to P^1 .
//
// It returns f, g, and n such that j = n*f^a/g^b
///////////////////////////////////////////////////////////////
// Optional: D -- study j-D instead. (We only care about D - 12^3).
// 	     anti -- anti-symplectic case.
///////////////////////////////////////////////////////////////

getPolys := function(c,N : D := 0, anti := false)
	P<s,t> := PolynomialRing(Rationals(),2);
	j := getjInv(c,N : anti := anti);

	J := Evaluate(j,s/t)-D;
	  f := SquareFreeFactorization(Numerator(J))[1][1];	
	    n := Rationals()!(Numerator(J)/f^d)
		where d is (D eq 12^3 select 2 else 3);
	  g := SquareFreeFactorization(Denominator(J))[1][1];
	
	return [f,g,n];
end function;


 
////////////////////////////////////////////////////////////////////
// INPUT: An elliptic curve c, an integer N, a prime p, k = 1 or 2 
// corresponding to the residue classes [x,1] and [1,px]
//
// OUTPUT: A tuple <F,G,N,V> where
//	   N*F^d/G^e is the map j:P^1 = X_c(N) \to X(1) 
//		restricted to the residue class R and 
//	   V is the valuation at p of N
//
////////////////////////////////////////////////////////////////////
// Optional: D -- study j-D instead. (We only care about D - 12^3).
// 	     anti -- anti-symplectic case.
////////////////////////////////////////////////////////////////////


getPolysP := function(c,N,p,k : D := 0, anti := false)
	P<s,t> := PolynomialRing(Rationals(),2);
	j := getjInv(c,N : anti := anti);

	PZ<x> := PolynomialRing(Rationals());
	R := k eq 1 select [x,1] else [1,p*x];

	J := Evaluate(j,s/t) - D;
	  f := SquareFreeFactorization(Numerator(J))[1][1];		
	    fa := Evaluate(f, R);
	  g := SquareFreeFactorization(Denominator(J))[1][1];
	    ga := Evaluate(g, R);
	  n := Rationals()!(Numerator(J)/f^d)
	      	    where d is (D eq 12^3 select 2 else 3);
	    	       

	return <  PZ!fa/af , 
	       	  PZ!ga/ag ,
		   n*af^d/ag^e  ,
	       	   Valuation(n*af^d/ag^e,p)
		   where af is 
		   	 LeadingCoefficient(fa)
		   where ag is 
		   	 LeadingCoefficient(ga)
		   where d is (D eq 12^3 select 2 else 3)
		   where e is (N eq 2    select 2 else 5 )
	       >;

end function;


///////////////////////////////////////////////////////
// This code creates the routines necessary for the 
// local tests of section 6 of the paper `Primitive
// Integral Solutions to x^2 + y^3 = z^10' by David
// Brown
///////////////////////////////////////////////////////

  // this stuff is just for testing and should disappear.
  P<t> := PolynomialRing(Rationals());
  f := 3*((1/2)*t^5 + 3*t + 1/8);

//  load "local_2_get_modular_equations";

///////////////////////////////////////////////////////
// rootData
///////////////////////////////////////////////////////
//
// INPUT: A polynomial f(x) \in \Q[x], and a prime p
//
// OUTPUT: for every irreducible factor of f in Z_p, an integer 
// 	       	    a such that for any root b, b-a has `leading 
//		    term' outside of Z_p. For linear factors this 
// 		    returns `Infinity' 
//
//	   `Leading term' means leading term in a pi-adic expansion, 
//   	   where pi is a uniformizer of the splitting field of the factor
//
// The output is of the form < <a, [<v,m>]> ... >
//   where a 
//   where v is the valuation at p of the `leading term'
//   where m is the multiplicity of the root in f
///////////////////////////////////////////////////////

rootData := function(f,p : prec := 1000);
  R := pAdicField(p,prec);
  P<t> := PolynomialRing(R);
  f := P!f;

  if not IsIrreducible(f) then
    return < $$(g[1],p) : g in Factorization(f) >;
  end if;

  if Degree(f) eq 1 then
    return <Infinity(), ValuationsOfRoots(f)>;
  end if;

  N := ValuationsOfRoots(f)[1][1];
  if not IsIntegral(N) or N lt 0 then
    return <0, ValuationsOfRoots(f)>;
  end if;

  N := Numerator(N); // This just converts it from a rational number to an integer.

  if exists(a){a : a in [1..p-1] | ValuationsOfRoots( Evaluate(f,t + R!(p^N*a) ) ) [1][1] gt N} then
    return <b, ValuationsOfRoots(Evaluate(f,t+b))>
    	   where b is p^N*a +  $$(Evaluate(f,t+R!(p^N*a)) , p)[1];
  else
    return <0, ValuationsOfRoots(f)>;
  end if;
end function;


/////////////////////////////////////////////////////////////////
// localTest
/////////////////////////////////////////////////////////////////
//
// INPUT: An elliptic curve E, a prime p and an integer N
//	  and k = 1 or 2, picking out the residue class 
//	  [x:1] or [1:px]
//
// OUTPUT: All possible valuations of j(E') for E'[N]
// 	   (anti)symplectically isomorphic to E[N] 	 
//  
//	   (Strictly speaking, one uses this data directly to compute
//	   v(j(E')) as described in section 6 of my paper).
/////////////////////////////////////////////////////////////////
//
// Optional: prec (increase this when p-adic factorization
// 	     	  fails).
//	     anti -- this switches to the antisymplectic case
//
/////////////////////////////////////////////////////////////////

localTest := function(E,N,p,k : D := 0, prec := 1000, anti := false)
  da := getPolysP(E,N,p,k : D := D, anti := anti);
  return  <rootData(da[1],p : prec := prec) , 
	   rootData(da[2],p : prec := prec) , 
	   da[4]>;
end function;




==> code/chabautyNecessities <==
///////////////////////////////////////////////////////////////////////
// This Magma code constructs the object of sections 3 and 4 of
// "Primitive integral solutions to X^2 + y^3 = z^10" by David Brown
//
// These are necessary for the elliptic Chabauty computation of section 5
// and is called by the other MAGMA routines.
///////////////////////////////////////////////////////////////////////

QQ := Rationals();
ZZ := Integers();
P<t> := PolynomialRing(QQ);


//////////////////////////////////////////////////////////////////////
// This is the defining polynomial of the number field K_j
//////////////////////////////////////////////////////////////////////

    fj :=  (t^2 + 250*t + 3125)^3  - j*t^5;


    //////////////////////////////////////////////////////////////////////
    // Need to factor because in the CM case fj may not be irreducible.
    // In the j = 12^3 case there are multiple isogenies, defined over different
    // fields. The second choice of field gives a curve of rank 0.
    //////////////////////////////////////////////////////////////////////

    Fj := j eq 12^3 select Factorization(fj)[2][1]
        else Factorization(fj)[1][1];


    //////////////////////////////////////////////////////////////////////
    // This creates the number field K_j 
    //
    // An elliptic curve E with j(E) = j has a 5 isogeny over this field.
    //////////////////////////////////////////////////////////////////////

    Kj := NumberField(Fj);

//////////////////////////////////////////////////////////////////////
// This creates the elliptic curve X_{E_0} over QQ and
// for a given j creates it over K_E
//////////////////////////////////////////////////////////////////////

EQ<x,y,z> := EllipticCurve(t*(t^2  + (-3)*22*t +(-3)^2*125));
Ej := BaseExtend(EQ,Kj);


    //////////////////////////////////////////////////////////////////////
    // This creates the canonical point on X_E_0(K_E) coming from the 
    // 5-isogeny of E over K_j. 
    //
    // For this to work j(E) must be in the image of -3z^2 + 12^3
    //////////////////////////////////////////////////////////////////////

    bool, z0 := IsSquare((j-12^3)/(-3));
    if bool then
      canPts :=  {@Ej![ -3*Kj.1, 9*z0*Kj.1^3/p1 ,1]
          where p1 is Evaluate(t^2 - 500*t - 15625, Kj.1)@};
      else
          canPts := {@@};
    end if;


//////////////////////////////////////////////////////////////////////
// Create the map X_E_0 \to X_E_0,Delta
//-- extend the map to cover pts at infty etc TODO
//////////////////////////////////////////////////////////////////////

    P1<Z,W> := ProjectiveSpace(Rationals(),1);
    jp0 := map< EQ -> P1 | [-3*y*(X^2 - 500*X*z - 15625*z^2), x^3  ] 
    	   where X is x/-3  >;
    jp0 := Extend(jp0);


    //////////////////////////////////////////////////////////////////////
    // Base Extend to K_j
    //-- Extend the map to cover .. TODO
    //////////////////////////////////////////////////////////////////////

    P1j<Z,W> := ProjectiveSpace(Kj,1);
    jp := map< Ej -> P1 | [ -3*y*(X^2 - 500*X*z - 15625*z^2), x^3  ] 
       	    where X is x/-3  >;
    jp := Extend(jp);

    //////////////////////////////////////////////////////////////////////
    // Create the map X_E_0,Delta \to X(1)
    //////////////////////////////////////////////////////////////////////

    sp := map<P1 -> P1 | [-3*Z^2 + 12^3*W^2, W^2]>;
    sp := Extend(sp);

//////////////////////////////////////////////////////////////////////
// Create the MWmap
//////////////////////////////////////////////////////////////////////

G := AbelianGroup([6,0]);
gs := [Ej![45 , 90 , 1] , canPts[1]] ; 
mwMap := map<G->Ej|g:->&+[c[i]*gs[i]:i in [1..#gs]] where c:=Eltseq(g)>;





==> code/chabauty_0 <==
////////////////////////////////////////////////////////////////////
// This Magma code does the elliptic Chabauty computations necessary
// for section 5 of  "Primitive integral solutions to X^2 + y^3 = z^10" 
// by David Brown, in the case of j = -13824
////////////////////////////////////////////////////////////////////

////////////////////////////////////////////////////////////////////
// Construct the number fields, curves, maps, etc necessary.
////////////////////////////////////////////////////////////////////

j := 0;
load "chabautyNecessities";


////////////////////////////////////////////////////////////////////
// Do a two descent.
////////////////////////////////////////////////////////////////////

//RankBound(Ej); // Returns 1


////////////////////////////////////////////////////////////////////
// Do the elliptic Chabauty computation. 
// 7 is the first prime that works.
////////////////////////////////////////////////////////////////////

p := 19; 
bound, found, index, cosets := Chabauty(mwMap,jp,p : Aux := {13});

    // bound returns 10
    // found returns 10
       found := SetToIndexedSet(found);
    // index returns 2



////////////////////////////////////////////////////////////////////
// Since the index is 40. We need to check that G \subset  E(K) has 
// index coprime to 40
////////////////////////////////////////////////////////////////////

    ////////////////////////////////////////////////////////////////////
    // Check 2-saturation
    // Q is the canonical point of infinite order
    // T is the non-trivial two torsion point
    // 
    // We don't need to worry about 3-torsion because 5 is prime to 3
    ////////////////////////////////////////////////////////////////////


    {#DivisionPoints(P,2)
        where P is a*Q + b*T
        where Q is gs[2]
        where T is 3*gs[1]:
        a in [1..1], b in [0..1] };
	  
    // Returns {0}, so G is 2-saturated


////////////////////////////////////////////////////////////////////
// Check the images of the found points and see if they correspond 
// to primitive solutions to x^2 + y^3 = z^10
////////////////////////////////////////////////////////////////////

images := {@ sp(jp(mwMap( pt ))) : pt in found @};

    // returns no new j Invariants.

bound;

==> code/chabauty_13824 <==
////////////////////////////////////////////////////////////////////
// This Magma code does the elliptic Chabauty computations necessary
// for section 5 of  "Primitive integral solutions to X^2 + y^3 = z^10" 
// by David Brown, in the case of j = -13824
////////////////////////////////////////////////////////////////////

////////////////////////////////////////////////////////////////////
// Construct the number fields, curves, maps, etc necessary.
////////////////////////////////////////////////////////////////////

j := -13824;
load "chabautyNecessities";


////////////////////////////////////////////////////////////////////
// Do a two descent.
////////////////////////////////////////////////////////////////////

RankBound(Ej); // Returns 1


////////////////////////////////////////////////////////////////////
// Do the elliptic Chabauty computation. 
// 7 is the first prime that works.
////////////////////////////////////////////////////////////////////

p := 7; 
bound, found, index, cosets := Chabauty(mwMap,jp,p);

    // bound returns 8
    // found returns 8
       found := SetToIndexedSet(found);
    // index returns 40



////////////////////////////////////////////////////////////////////
// Since the index is 40. We need to check that G \subset  E(K) has 
// index coprime to 40
////////////////////////////////////////////////////////////////////

    ////////////////////////////////////////////////////////////////////
    // Check 2-saturation
    // Q is the canonical point of infinite order
    // T is the non-trivial two torsion point
    // 
    // We don't need to worry about 3-torsion because 5 is prime to 3
    ////////////////////////////////////////////////////////////////////


    {#DivisionPoints(P,2)
        where P is a*Q + b*T
        where Q is gs[2]
        where T is 3*gs[1]:
        a in [1..1], b in [0..1] };
	  
    // Returns {0}, so G is 2-saturated
    
    ////////////////////////////////////////////////////////////////////	
    // Check 5-saturation
    // Only need to check P because 5 is prime to the order of the torsion
    ////////////////////////////////////////////////////////////////////

    #DivisionPoints(Q,5)
	where Q is gs[2];

    // Returns 0, so G is 5-saturated.

////////////////////////////////////////////////////////////////////
// Check the images of the found points and see if they correspond 
// to primitive solutions to x^2 + y^3 = z^10
////////////////////////////////////////////////////////////////////

images := {@ sp(jp(mwMap( pt ))) : pt in found @};

    // returns no new j Invariants.

==> code/local_2_get_modular_equations <==
///////////////////////////////////////////////////////
// This code creates the explicit equations for the maps 
// X_E(5) \to X(1) necessary for the 
// local tests of section 6 of the paper `Primitive
// Integral Solutions to x^2 + y^3 = z^10' by David
// Brown
///////////////////////////////////////////////////////

QQ := Rationals();
ZZ := Integers();
P<t> := PolynomialRing(QQ);

load "local_1_get_elliptic_curves";


////////////////////////////////////////////////////////////////
// INPUT: an elliptic curve c and an integer N
//
////////////////////////////////////////////////////////////////
// OUTPUT: The (affine piece of) the map X_c(N) to P^1  
// 	   (Symplectic case)
////////////////////////////////////////////////////////////////

getjInvSymp := function(c,N)
	////////////////////////////////////////////////////////
	// This gets the input to the RubSilv rouutine
	////////////////////////////////////////////////////////

	j := jInvariant(c);
	J := j/12^3;

	eqn := Coefficients(WeierstrassModel(c));
	A := eqn[4];
	B := eqn[5];

	////////////////////////////////////////////////////////
	// Get the X_E(N) \to X(1) equations
	////////////////////////////////////////////////////////
	a,b := RubinSilverbergPolynomials(N,J);

	////////////////////////////////////////////////////////
	// Make the universal elliptic curve, with parameter T
	////////////////////////////////////////////////////////
	P := Parent(a);
	Q<T> := FieldOfFractions(P);

	e := EllipticCurve([A*Q!a,B*Q!b]);

	////////////////////////////////////////////////////////
	// get the universal j-invariant 
	////////////////////////////////////////////////////////
	j := jInvariant(e);

	////////////////////////////////////////////////////////
        // Break it up
	////////////////////////////////////////////////////////
	num := Numerator(j);
	den := Denominator(j);	

	return j, num, den;
end function;



//////////////////////////////////////////////////////////////
// Helper routines for computing equations for the 
// anti-symplectic twist X_c(N)^- \to X(1)
//////////////////////////////////////////////////////////////

//////////////////////////////////////////////////////////////
// 1) Compute a number field K such that 
//    E has an isogeny over K
//////////////////////////////////////////////////////////////

twoIsogenyPolynomial := function(c)
	j := jInvariant(c);
	phi := AtkinModularPolynomial(2);
	return Evaluate(phi,[t,j]);
end function;


twoIsogenyField := function(c)
	j := jInvariant(c);
	phi := AtkinModularPolynomial(2);
	return K, K.1 where K is NumberField(f) where f is Factorization(Evaluate(phi,[t,j]))[1][1];
end function;


///////////////////////////////////////////////////
// Subroutine *Mobius*: 
//  Input: two triples of points in A^1
//  Output: the corresponding map P^1 to P^1
//  (the affine polynomial at least)
///////////////////////////////////////////////////

mobius := function(e,j)
     M := Matrix(3,4,
       [[e[1],1,-j[1]*e[1],-j[1]],
        [e[2],1,-j[2]*e[2],-j[2]],
        [e[3],1,-j[3]*e[3],-j[3]] ]
     );
     
     b := Basis(NullspaceOfTranspose(M))[1];
       P<t> := PolynomialRing(BaseRing(Parent(b)));
     return (b[1]*t + b[2])/(b[3]*t + b[4]);
end function;


///////////////////////////////////////////////////
// getAntiSymplectic:
///////////////////////////////////////////////////
// Input: elliptic curve c, an integer N. 
//	    		    (only N = 5 is implemented)
// Output: equations for the anti-symplectic twist
// 	   X_c'(N) of X(N)  
///////////////////////////////////////////////////

///////////////////////////////////////////////////
// Antisymplectic case
///////////////////////////////////////////////////
// The pre-computed polys are in the file `saved polys' under
// the name antiSympPolys; 
////////////////////////////////////////////////////////////

//restore "savedPolys"; // Uncomment this line if using 
	  		// precomputed polynomials.
antiSympPolys := [];    


getjInvAntiSymp :=  function(c : preCompute := false) 
    P<T> := PolynomialRing(Rationals());

  if not preCompute then

    //////////////////////////////////////////////////    
    // Get (and match up) the two torsion and 
    // two isogenies.
    //////////////////////////////////////////////////
    j := jInvariant(c);	      

    f := HyperellipticPolynomials(c);
        K := SplittingField(f);	      	      
	Q<t> := PolynomialRing(K);
	e := BaseExtend(c,K);
    F := Q!f;
        roots    := [r[1] : r in Roots(F)];
    	twoTors  := [e![r,0,1] : r in roots];
	twoIsogs := [TwoIsogeny(i) : i in twoTors];
	jInvsIsog := [jInvariant(Codomain(phi)) : phi in twoIsogs];
	
    //////////////////////////////////////////////////
    // Construct the canonical points on X_F(5), 
    // where F is the first isogenous curve
    //
    // Also, MAGMA v.2.13.6 has coercion issues... 
    //////////////////////////////////////////////////
    j,n,d := getjInvSymp(Codomain(twoIsogs[1]) , 5);
    canPts := {@0@};
	   _,can2 := HasRoot(n - jInvsIsog[2]*d);
	   	  _,m := IsIsomorphic(Parent(can2),K);
		  can2 := m(can2);	  
	     canPts := canPts join {@can2@};
	   _,can3 := HasRoot(n - jInvsIsog[3]*d);
	   	  _,m := IsIsomorphic(Parent(can3),K);
		  can3 := m(can3);
	     canPts := canPts join {@can3@};	   	      


    jQ :=  Evaluate(j,mobius(roots,canPts));
    return P!Numerator(jQ)/P!Denominator(jQ);

  else
    if exists(i){i : i in [1..#crvsAnti] | IsIsomorphic(c,crvsAnti[i])} 
    then
       return antiSympPolys[i];
    else
	return "Nothing precomputed for this curve";
    end if;
  end if;    	   
end function;


///////////////////////////////////////////////////////////////
// getjInvs -- auxiliary function combining the symp and anti 
// 	       symplectic cases.
///////////////////////////////////////////////////////////////

getjInv := function(c,N : anti := false, preCompute := true)
  return not anti select getjInvSymp(c,N)
  	 else getjInvAntiSymp(c : preCompute := preCompute);	 
end function;



///////////////////////////////////////////////////////////////
// This collects the (factors of the) homogeneous 
// polynomials defining the map X_c(N) \to P^1 .
//
// It returns f, g, and n such that j = n*f^a/g^b
///////////////////////////////////////////////////////////////
// Optional: D -- study j-D instead. (We only care about D - 12^3).
// 	     anti -- anti-symplectic case.
///////////////////////////////////////////////////////////////

getPolys := function(c,N : D := 0, anti := false)
	P<s,t> := PolynomialRing(Rationals(),2);
	j := getjInv(c,N : anti := anti);

	J := Evaluate(j,s/t)-D;
	  f := SquareFreeFactorization(Numerator(J))[1][1];	
	    n := Rationals()!(Numerator(J)/f^d)
		where d is (D eq 12^3 select 2 else 3);
	  g := SquareFreeFactorization(Denominator(J))[1][1];
	
	return [f,g,n];
end function;


 
////////////////////////////////////////////////////////////////////
// INPUT: An elliptic curve c, an integer N, a prime p, k = 1 or 2 
// corresponding to the residue classes [x,1] and [1,px]
//
// OUTPUT: A tuple <F,G,N,V> where
//	   N*F^d/G^e is the map j:P^1 = X_c(N) \to X(1) 
//		restricted to the residue class R and 
//	   V is the valuation at p of N
//
////////////////////////////////////////////////////////////////////
// Optional: D -- study j-D instead. (We only care about D - 12^3).
// 	     anti -- anti-symplectic case.
////////////////////////////////////////////////////////////////////
// This does the same as getPoly but makes everything 
// p-integral and inserts the residue classes.
//	(so that we get one variable polynomials which are prepared
//	 for the local test)
//
// It also returns the leading coefficients and their valuations.
////////////////////////////////////////////////////////////////////
// TODO: Strictly speaking, there should be a function that gets 
// 	 extra data at the end.
////////////////////////////////////////////////////////////////////

getPolysP := function(c,N,p,k : D := 0, anti := false)
	P<s,t> := PolynomialRing(Rationals(),2);
	j := getjInv(c,N : anti := anti);

	PZ<x> := PolynomialRing(Rationals());
	R := k eq 1 select [x,1] else [1,p*x];

	J := Evaluate(j,s/t) - D;
	  f := SquareFreeFactorization(Numerator(J))[1][1];		
	    fa := Evaluate(f, R);
	  g := SquareFreeFactorization(Denominator(J))[1][1];
	    ga := Evaluate(g, R);
	  n := Rationals()!(Numerator(J)/f^d)
	      	    where d is (D eq 12^3 select 2 else 3);
	    	       

	return <  PZ!fa/af , 
	       	  PZ!ga/ag ,
		   n*af^d/ag^e  ,
	       	   Valuation(n*af^d/ag^e,p)
		   where af is 
		   	 LeadingCoefficient(fa)
		   where ag is 
		   	 LeadingCoefficient(ga)
		   where d is (D eq 12^3 select 2 else 3)
		   where e is (N eq 2    select 2 else 5 )
	       >;

end function;




==> code/local_3_final_test <==
///////////////////////////////////////////////////////
// This code creates the routines necessary for the 
// local tests of section 6 of the paper `Primitive
// Integral Solutions to x^2 + y^3 = z^10' by David
// Brown
///////////////////////////////////////////////////////

  // this stuff is just for testing and should disappear.
  P<t> := PolynomialRing(Rationals());
  f := 3*((1/2)*t^5 + 3*t + 1/8);

  load "local_2_get_modular_equations";


///////////////////////////////////////////////////////
// rootData 
///////////////////////////////////////////////////////
//
// INPUT: A polynomial f(x) \in \Q[x], and a prime p
//
// OUTPUT: for every irreducible factor of f in Z_p, an integer 
// 	       	    a such that for any root b, b-a has `leading 
//		    term' outside of Z_p. For linear factors this 
// 		    returns `Infinity' 
//
//	   `Leading term' means leading term in a pi-adic expansion, 
//   	   where pi is a uniformizer of the splitting field of the factor
//
// The output is of the form < <a, [<v,m>]> ... >
//   where a 
//   where v is the valuation at p of the `leading term'
//   where m is the multiplicity of the root in f
///////////////////////////////////////////////////////

rootData := function(f,p : prec := 1000);
  R := pAdicField(p,prec);
  P<t> := PolynomialRing(R);
  f := P!f;

  if not IsIrreducible(f) then
    return < $$(g[1],p) : g in Factorization(f) >;
  end if;

  if Degree(f) eq 1 then
    return <Infinity(), ValuationsOfRoots(f)>;
  end if;

  N := ValuationsOfRoots(f)[1][1];
  if not IsIntegral(N) or N lt 0 then
    return <0, ValuationsOfRoots(f)>;
  end if;

  N := Numerator(N); // This just converts it from a rational number to an integer.

  if exists(a){a : a in [1..p-1] | ValuationsOfRoots( Evaluate(f,t + R!(p^N*a) ) ) [1][1] gt N} then
    return <b, ValuationsOfRoots(Evaluate(f,t+b))>
    	   where b is p^N*a +  $$(Evaluate(f,t+R!(p^N*a)) , p)[1];
  else
    return <0, ValuationsOfRoots(f)>;
  end if;
end function;


/////////////////////////////////////////////////////////////////
// localTest
/////////////////////////////////////////////////////////////////
//
// INPUT: An elliptic curve E, a prime p and an integer N
//	  and k = 1 or 2, picking out the residue class 
//	  [x:1] or [1:px]
//
// OUTPUT: All possible valuations of j(E') for E'[N]
// 	   (anti)symplectically isomorphic to E[N] 	 
//  
//	   (Strictly speaking, one uses this data directly to compute
//	   v(j(E')) as described in section 6 of my paper).
/////////////////////////////////////////////////////////////////
//
// Optional: prec (increase this when p-adic factorization
// 	     	  fails).
//	     anti -- this switches to the antisymplectic case
//
/////////////////////////////////////////////////////////////////

localTest := function(E,N,p,k : D := 0, prec := 1000, anti := false)
  da := getPolysP(E,N,p,k : D := D, anti := anti);
  return  <rootData(da[1],p : prec := prec) , 
	   rootData(da[2],p : prec := prec) , 
	   da[4]>;
end function;

